Lithium detection in red supergiant stars of the Perseus complex

We present the first systematic study of lithium abundance in a chemically homogeneous sample of 27 red supergiants (RSGs) in the young Perseus complex. For these stars, accurate stellar parameters and detailed chemical abundances of iron and iron peak, CNO, alpha, light and neutron-capture elements have been already obtained by means of high resolution optical and near-infrared spectroscopy. The observed RSGs have half-solar metallicity, 10-30 Myr age, bolometric luminosities in the 10$^4$-10$^5$ L$_{\odot}$ range and likely mass progenitors in the 9-14 M$_{\odot}$ range. We detected the optical Li I doublet in eight out of the 27 observed K and M type RSGs, finding relatively low A(Li)$<$1.0 dex abundances, while for the remaining 19 RSGs upper limits of A(Li)$<$-0.2 dex have been set. Warmer and less luminous (i.e. likely less massive) as well as less mixed (i.e. with lower [C/N] and $^{12}$C/$^{13}$C depletion) RSGs with Li detection show somewhat higher Li abundances. In order to explain Li detection in $\sim$30\% of the observed RSGs, we speculate that some stochasticity and a scenario where Li was not completely destroyed in the convective atmospheres and/or a secondary production took place during the post-Main Sequence evolution, should be at work.

==> tab2.tex <==
\begin{table}[!h]
\centering
%\tiny
\scriptsize
\addtolength{\tabcolsep}{-3.3pt}
\caption{}
\begin{tabular}{|l|cc|c|ccc|c|c|}
\hline
ID & RA & Dec & parallax & G & BP & RP & RV & v sin($i$) \\
  & \multicolumn{2}{c|}{deg} & mas & \multicolumn{3}{c|}{Gaia EDR3} & \multicolumn{2}{c|}{km s$^{-1}$} \\
\hline
P2    & 36.316781 & 56.609815 &  0.442422 &   6.14 &   6.30 &   5.84 & -43.42 &  55.17  \\  
P3    & 35.480976 & 57.242911 &  0.450917 &   6.21 &   6.57 &   5.69 & -43.66 &  19.82  \\  
P4    & 32.871634 & 57.645542 &  0.524263 &   6.26 &   6.46 &   5.93 & -34.48 &  33.41  \\  
P5    & 34.215479 & 57.055240 &  0.429048 &   6.37 &   6.53 &   6.10 & -43.93 &  70.68  \\  
P6    & 34.768547 & 57.135494 &  0.434804 &   6.44 &   6.70 &   5.99 & -41.91 &  33.98  \\  
P7    & 34.808087 & 57.169226 &  0.411042 &   6.51 &   6.79 &   6.04 & -52.75 &  50.58  \\  
P8    & 37.972397 & 57.697637 &  0.370487 &   6.76 &   7.24 &   6.11 & -44.80 &  30.46  \\  
P9    & 35.751769 & 57.387001 &  0.438911 &   6.79 &   7.17 &   6.22 & -48.78 &  31.61  \\  
P11   & 37.493983 & 57.820709 &  0.390141 &   6.92 &   7.43 &   6.26 & -48.80 &  16.51  \\  
P13   & 34.193289 & 57.029347 &  0.413678 &   7.30 &   7.42 &   7.07 & -41.78 &  54.51  \\  
P14   & 33.994564 & 58.293614 &  0.404561 &   7.34 &   7.82 &   6.68 & -47.16 &  15.81  \\  
P17   & 38.386605 & 57.537425 &  0.447177 &   7.81 &   8.19 &   7.26 & -42.31 &  55.42  \\  
P18   & 35.502397 & 57.144959 &  0.413029 &   7.95 &   8.14 &   7.64 & -43.76 &  31.76  \\  
P19   & 38.220315 & 57.929345 &  0.421863 &   7.99 &   8.56 &   7.27 & -42.54 &  32.64  \\  
P20   & 39.658666 & 57.816982 &  0.356374 &   8.04 &   8.39 &   7.53 & -37.05 &  33.70  \\  
P21   & 34.617316 & 57.208368 &  0.421770 &   8.10 &   8.26 &   7.81 & - 8.30 &  60.80  \\  
P23   & 34.793528 & 57.130579 &  0.407938 &   8.36 &   8.57 &   7.98 & -37.67 &  93.37  \\  
P26   & 35.461710 & 57.386563 &  0.372927 &   8.46 &   8.79 &   7.92 & -41.81 & 102.52  \\  
P27   & 35.142196 & 56.329950 &  0.387312 &   8.49 &   8.62 &   8.23 & -41.12 &  80.71  \\  
P28   & 33.777066 & 56.926520 &  0.393302 &   8.52 &   8.77 &   8.10 & -32.96 &  33.14  \\  
P30   & 37.431733 & 58.125222 &  0.420213 &   8.68 &   9.10 &   8.08 & -49.72 &  13.69  \\  
P31   & 35.570651 & 57.271929 &  0.389598 &   8.70 &   8.86 &   8.31 & -47.80 &  33.54  \\  
P32   & 36.495801 & 56.657906 &  0.668790 &   8.80 &   8.97 &   8.49 & -50.14 &  97.55  \\  
P36   & 36.193054 & 57.464203 &  0.408014 &   9.01 &   9.31 &   8.53 & -47.95 & 105.03  \\  
P37   & 34.053790 & 57.616172 &  0.520453 &   9.07 &   9.64 &   8.35 & -37.60 &  16.95  \\  
P42   & 34.788511 & 57.135087 &  0.400982 &   9.18 &   9.39 &   8.81 & -49.95 & 101.56  \\  
P52   & 38.907649 & 57.487018 &  0.408809 &   9.39 &   9.66 &   8.95 & -57.79 &  55.84  \\  
P54   & 33.150279 & 58.098358 &  0.395671 &   9.41 &   9.55 &   9.14 & -50.28 & 105.03  \\  
P61   & 35.873129 & 58.963489 &  0.435709 &   9.49 &   9.85 &   8.94 & -41.00 & 107.05  \\  
P64   & 37.902227 & 57.753128 &  0.390878 &   9.68 &  10.14 &   9.05 & -46.20 & 100.16  \\  
N6    & 29.515885 & 60.391091 &  0.322135 &   7.73 &   8.28 &   7.00 & -36.60 &  23.80  \\  
N18   & 22.968979 & 61.523579 &  0.373128 &   7.67 &   8.37 &   6.83 & -45.00 &  12.96  \\  
N23   & 21.142584 & 62.788709 &  0.339883 &   8.39 &   8.97 &   7.64 & -52.60 &  38.76  \\  
N25   & 26.734947 & 60.669761 &  0.289411 &   7.42 &   7.68 &   6.98 & -37.30 &  28.90  \\  
N35   & 26.483806 & 61.234807 &  0.352103 &   8.62 &   9.15 &   7.92 & -28.80 &  32.85  \\  
N36   & 26.542574 & 61.442571 &  0.368448 &   8.81 &   9.30 &   8.15 & -32.30 &  29.38  \\  
N52   & 25.600511 & 63.429080 &  0.294924 &   8.27 &   8.72 &   7.63 & -69.00 &  11.60  \\  
N62   & 23.308343 & 60.686434 &  0.344024 &   7.15 &   7.33 &   6.85 & -46.20 &  33.40  \\  
N70   & 22.824957 & 63.347572 &  0.399289 &   7.31 &   7.64 &   6.80 & -40.10 &  32.44  \\  
AS19  & 41.714378 & 57.733797 &  0.336350 &   7.25 &   7.75 &   6.57 & -39.40 &  32.06  \\  
AS21  & 41.851031 & 57.677103 &  0.415104 &   7.79 &   8.30 &   7.12 & -40.10 &  34.11  \\  
IC6   & 42.783226 & 60.417740 &  0.414680 &   7.21 &   7.41 &   6.81 & -57.20 & 101.47  \\  
IC14  & 36.943605 & 60.452751 &  0.479554 &   9.57 &  10.48 &   8.62 & -53.00 &  32.79  \\  
IC17  & 38.205913 & 61.378354 &  0.442391 &   7.88 &   8.33 &   7.25 & -42.50 & 103.62  \\  
IC30  & 33.358386 & 60.542677 &  0.384439 &   9.48 &  10.66 &   8.40 & -44.90 &  19.32  \\  
IC31  & 32.932952 & 60.712360 &  0.298858 &   7.98 &   8.81 &   7.06 & -40.10 &  67.99  \\  
\hline\hline
\end{tabular}
\label{tab_obs_all} 
\end{table}


==> tab_lines.tex <==
\begin{table}
\centering
%\tiny
\addtolength{\tabcolsep}{-2.25pt}
\caption{}
\label{tab_obs}
\begin{tabular}{|c|c|}
\hline
  & $\lambda$ & 
\hline

\hline\hline
\end{tabular}
Note: Solar reference for [Fe/H] is  from \citet{Grevesse98}.
\end{table}




%slow
%4267.2  C II *multipletto  fast
%4387.9  He                 fast
%4437.5  He
%4471.5  He                 fast
%4512.6  Al II
%4552.6  Si II
%4567.8  Si II
%4591.0  O II
%4630.5  N II
%4661.6  O II
%4921.9 He                  only fast


